Cosmological constraints from standardized non-CMB observations

The current expansion of the Universe has been observed to be accelerating, and the widely accepted spatially-flat concordance model of general relativistic cosmology attributes this phenomenon to a constant dark energy, a cosmological constant, which is measured to comprise about 70% of the total energy budget of the current Universe. However, observational discrepancies and theoretical puzzles have raised questions about this model, suggesting that alternative cosmological models with non-zero spatial curvature and/or dark energy dynamics might provide better explanations. To explore these possibilities, we have conducted a series of studies using standardized, lower-redshift observations to constrain six different cosmological models with varying degrees of flatness and dark energy dynamics. Through comparing these observations with theoretical predictions, we aim to deepen our understanding of the evolution of the Universe and shed new light on its mysteries. Our data provide consistent cosmological constraints across all six models, with some suggesting the possibility of mild dark energy dynamics and slight spatial curvature. However, these joint constraints do not rule out the possibility of dark energy being a cosmological constant and the spatial hypersurfaces being flat. Overall, our findings contribute to the ongoing efforts to refine our understanding of the Universe and its properties, and suggest that multiple cosmological models remain viable.

==> chapter12.tex <==
% +--------------------------------------------------------------------+
% | Sample Chapter 12
% +--------------------------------------------------------------------+

\cleardoublepage

% +--------------------------------------------------------------------+
% | Replace "This is Chapter 12" below with the title of your chapter.
% | LaTeX will automatically number the chapters.                      
% +--------------------------------------------------------------------+

\chapter{This is Chapter 12}
\label{makereference12}


==> dedication.tex <==
% +--------------------------------------------------------------------+
% | Dedication Page (Optional)
% +--------------------------------------------------------------------+

\newpage
\vspace*{0.9cm}
\begin{center}
{\bf \Huge Dedication}
\end{center}

\setlength{\baselineskip}{0.8cm}

%\pdfbookmark[0]{Dedication}{PDF_Dedication}

% +--------------------------------------------------------------------+
% | Enter the text for your dedication in the space below this box.    
% +--------------------------------------------------------------------+

Enter the text for your Dedication page in the dedication.tex file.  The Dedication page is optional.  If you wish to remove it, see the comments in the etdrtemplate.tex file.


==> nomenclature.tex <==
% +--------------------------------------------------------------------+
% | Nomenclature Page (Optional)
% +--------------------------------------------------------------------+

\newpage
\vspace*{0.9cm}
\begin{center}
{\bf \Huge Nomenclature}
\end{center}

\setlength{\baselineskip}{0.8cm}

%\pdfbookmark[0]{Nomenclature}{PDF_Nomenclature}

% +--------------------------------------------------------------------+
% | Enter the text for your dedication in the space below this box.    
% +--------------------------------------------------------------------+

Enter the text for your Nomenclature page in the nomenclature.tex file.  The Nomenclature page is optional.  If you wish to remove it, see the comments in the etdrtemplate.tex file.


==> preface.tex <==
% +--------------------------------------------------------------------+
% | Preface (Optional)
% +--------------------------------------------------------------------+

\newpage
\vspace*{0.9cm}
\begin{center}
{\bf \Huge Preface}
\end{center}

\setlength{\baselineskip}{0.8cm}

%\pdfbookmark[0]{Preface}{PDF_Preface}

% +--------------------------------------------------------------------+
% | Enter text of your Preface in the space below this box.            
% +--------------------------------------------------------------------+

Enter the text for your Preface page in the preface.tex file. The Preface page is optional.  If you wish to remove it, see the comments in the etdrtemplate.tex file.

